A Transfer Attack to Image Watermarks

Watermark has been widely deployed by industry to detect AI-generated images. The robustness of such watermark-based detector against evasion attacks in the white-box and black-box settings is well understood in the literature. However, the robustness in the no-box setting is much less understood. In this work, we propose a new transfer evasion attack to image watermark in the no-box setting. Our transfer attack adds a perturbation to a watermarked image to evade multiple surrogate watermarking models trained by the attacker itself, and the perturbed watermarked image also evades the target watermarking model. Our major contribution is to show that, both theoretically and empirically, watermark-based AI-generated image detector based on existing watermarking methods is not robust to evasion attacks even if the attacker does not have access to the watermarking model nor the detection API. Our code is available at: https://github.com/hifi-hyp/Watermark-Transfer-Attack.

==> ethic.tex <==
\section{Ethics Considerations and Compliance with the Open Science Policy}
In this paper, we study a transfer attack to image watermarks, demonstrating both empirically and theoretically that current watermarking methods can be compromised and are not robust in the no-box setting. While our primary focus is on understanding the vulnerabilities in image watermarking, our ultimate goal is to contribute to the development of more robust watermarks that better detect AI-generated images. We hope this research will inspire further exploration and innovation in this field. Additionally, we commit to making the code for our transfer attack publicly available after publication, in full compliance with the open science policy, to support transparency and further research.

